PAH emission in the proplyd HST10: what is the mechanism behind photoevaporation?

Proplyds are photodissociation region (PDR)-like cometary cocoons around young stars which are thought to originate through photo-evaporation of the central protoplanetary disk by external UV radiation from the nearby OB stars. This letter presents spatially resolved mid-infrared imaging and spectroscopy of the proplyd HST10 obtained with the VLT/VISIR instrument. These observations allow us to detect Polycyclic Aromatic Hydrocarbons (PAH) emission in the proplyd photodissociation region and to study the general properties of PAHs in proplyds for the first time. We find that PAHs in HST10 are mostly neutral and at least 50 times less abundant than typical values found for the diffuse ISM or the nearby Orion Bar. With such a low PAH abundance, photoelectric heating is significantly reduced. If this low abundance pertains also to the original disk material, gas heating rates could be too low to efficiently drive photoevaporation unless other processes can be identified. Alternatively, the model behind the formation of proplyds as evaporating disks may have to be revised.

==> Vicente_HST10_ApJL_astroph.bbl.tex <==
\begin{thebibliography}{}

\bibitem[Bally et al.(1998)]{Bally1998} Bally, J., Sutherland, 
R.~S., Devine, D., \& Johnstone, D.\ 1998, \aj, 116, 293 

\bibitem[Bally et al.(2000)]{Bally2000} Bally, J., O'Dell, C.~R., 
\& McCaughrean, M.~J.\ 2000, \aj, 119, 2919 

\bibitem[Bern{\'e} 
\& Tielens(2012)]{Berne2012} Bern{\'e}, O., \& Tielens, A.~G.~G.~M.\ 2012, Proceedings of the National Academy of Science, 109, 401 

\bibitem[Chen et al.(1998)]{Chen1998} Chen, H., Bally, J., 
O'Dell, C.~R., et al.\ 1998, \apjl, 492, L173 

\bibitem[Geers et 
al.(2007)]{Geers2007} Geers, V.~C., van Dishoeck, E.~F., Visser, R., et al.\ 2007, \aap, 476, 279 


\bibitem[Giard et 
al.(1994)]{Giard1994} Giard, M., Bernard, J.~P., Lacombe, F., Normand, P., \& Rouan, D.\ 1994, \aap, 291, 239 

\bibitem[Habing(1968)]{Habing1968} Habing, H.~J.\ 1968, \bain, 19, 
421 

\bibitem[Henney et al.(1996)]{Henney1996} Henney, W.~J., Raga, 
A.~C., Lizano, S., \& Curiel, S.\ 1996, \apj, 465, 216 

\bibitem[Henney 
\& Arthur(1998)]{Henney1998} Henney, W.~J., \& Arthur, S.~J.\ 1998, \aj, 116, 322 

\bibitem[Henney 
\& O'Dell(1999)]{Henney1999} Henney, W.~J., \& O'Dell, C.~R.\ 1999, \aj, 118, 2350 

\bibitem[Hester et al.(2004)]{Hester2004} Hester, J.~J., Desch, 
S.~J., Healy, K.~R., \& Leshin, L.~A.\ 2004, Science, 304, 1116 

\bibitem[Hillenbrand 
\& Hartmann(1998)]{Hillenbrand1998} Hillenbrand, L.~A., \& Hartmann, L.~W.\ 1998, \apj, 492, 540 

\bibitem[Hollenbach 
\& Tielens(1997)]{Hollenbach1997} Hollenbach, D.~J., \& Tielens, A.~G.~G.~M.\ 1997, \araa, 35, 179 

\bibitem[Joblin et 
al.(2010)]{Joblin2010} Joblin, C., Pilleri, P., Montillaud, J., et al.\ 2010, \aap, 521, L25 

\bibitem[Joblin 
\& Tielens(2011)]{Joblin2011} Joblin, C., \& Tielens, A.~G.~G.~M.\ 2011, EAS Publications Series, 46,  

\bibitem[Johnstone et al.(1998)]{Johnstone1998} Johnstone, D., 
Hollenbach, D., \& Bally, J.\ 1998, \apj, 499, 758 

\bibitem[Kamp 
\& Dullemond(2004)]{Kamp2004} Kamp, I., \& Dullemond, C.~P.\ 2004, \apj, 615, 991 

\bibitem[Lada 
\& Lada(2003)]{Lada2003} Lada, C.~J., \& Lada, E.~A.\ 2003, \araa, 41, 57 

\bibitem[Lada et al.(2004)]{Lada2004} Lada, C.~J., Muench, 
A.~A., Lada, E.~A., \& Alves, J.~F.\ 2004, \aj, 128, 1254 

\bibitem[Lagage et al.(2004)]{Lagage2004} Lagage, P.~O., Pel, 
J.~W., Authier, M., et al.\ 2004, The Messenger, 117, 12 

\bibitem[Menten et 
al.(2007)]{Menten2007} Menten, K.~M., Reid, M.~J., Forbrich, J., \& Brunthaler, A.\ 2007, \aap, 474, 515 

\bibitem[O'Dell et al.(1993)]{O'Dell1993} O'Dell, C.~R., Wen, Z., 
\& Hu, X.\ 1993, \apj, 410, 696 

\bibitem[O'Dell 
\& Wen(1994)]{O'Dell1994} O'Dell, C.~R., \& Wen, Z.\ 1994, \apj, 436, 194 

\bibitem[Oliveira et al.(2010)]{Oliveira2010} Oliveira, I., 
Pontoppidan, K.~M., Mer{\'{\i}}n, B., et al.\ 2010, \apj, 714, 778 

\bibitem[Pantin et al.(2005)]{Pantin2005} Pantin, E., Lagage, 
O.-P., Claret, A., et al.\ 2005, The Messenger, 119, 25 

\bibitem[Pantin(2010)]{Pantin2010} Pantin, E.\ 2010, Ph.D.~Thesis, 
 Infrared Observations of Circumstellar Disks and Exoplanets, Universit\'e de Paris Diderot, 2010

\bibitem[Pilleri et 
al.(2012)]{Pilleri2012} Pilleri, P., Montillaud, J., Bern{\'e}, O., \& Joblin, C.\ 2012, \aap, 542, A69 

\bibitem[Richling 
\& Yorke(1998)]{Richling1998} Richling, S., \& Yorke, H.~W.\ 1998, \aap, 340, 508 

\bibitem[Richling 
\& Yorke(2000)]{Richling2000} Richling, S., \& Yorke, H.~W.\ 2000, \apj, 539, 258 

\bibitem[St{\"o}rzer
\& Hollenbach(1998)]{Storzer1998} St{\"o}rzer, H., \& Hollenbach, D.\ 1998, \apj, 495, 853 

\bibitem[St{\"o}rzer 
\& Hollenbach(1999)]{Storzer1999} St{\"o}rzer, H., \& Hollenbach, D.\ 1999, \apj, 515, 669 

\bibitem[Sutherland(1997)]{Sutherland1997} Sutherland, R.~S.\ 1997, 
IAU Colloq.~163: Accretion Phenomena and Related Outflows, 121, 566 

\bibitem[Tielens et al.(1994)]{Tielens1994} Tielens, A.~G.~G.~M., 
McKee, C.~F., Seab, C.~G., \& Hollenbach, D.~J.\ 1994, \apj, 431, 321 

\bibitem[Tielens(2005)]{Tielens2005} Tielens, A.~G.~G.~M.\ 2005, 
The Physics and Chemistry of the Interstellar Medium, by 
A.~G.~G.~M.~Tielens, pp.~.~ISBN 0521826349.~Cambridge, UK: Cambridge 
University Press,  2005

\bibitem[Vasconcelos et 
al.(2011)]{Vasconcelos2011} Vasconcelos, M.~J., Cerqueira, A.~H., \& Raga, A.~C.\ 2011, \aap, 527, A86 

 \end{thebibliography}

